Deep Evidential Regression

Deterministic neural networks (NNs) are increasingly being deployed in safety critical domains, where calibrated, robust, and efficient measures of uncertainty are crucial. In this paper, we propose a novel method for training non-Bayesian NNs to estimate a continuous target as well as its associated evidence in order to learn both aleatoric and epistemic uncertainty. We accomplish this by placing evidential priors over the original Gaussian likelihood function and training the NN to infer the hyperparameters of the evidential distribution. We additionally impose priors during training such that the model is regularized when its predicted evidence is not aligned with the correct output. Our method does not rely on sampling during inference or on out-of-distribution (OOD) examples for training, thus enabling efficient and scalable uncertainty learning. We demonstrate learning well-calibrated measures of uncertainty on various benchmarks, scaling to complex computer vision tasks, as well as robustness to adversarial and OOD test samples.

==> area_chair.tex <==
Dear Area Chair, 

Thank you for the constructive comments from our Reviewers and for your careful consideration of our manuscript.

As the reviewers correctly point out, our approach provides a novel and scalable method for jointly learning continuous targets and the associated uncertainty, while not requiring OOD data during training nor sampling during inference. Because of this, our method will enable critical applications of uncertainty estimation to resource constrained environments, such as robotics. Furthermore, our method is directly applicable to learning supervised continuous targets, (e.g., robot control learning, temporal forecasting, depth estimation), a significant limitation of prior work on Dirichlet Prior Networks [24] and Evidential Deep Learning for Classification [32]. Finally, we demonstrate that our method yields highly calibrated uncertainties, that are superior to the widely-adopted method of dropout-based sampling [5] and on par with memory- and compute-intensive ensembles [21].

In response to our manuscript, the reviewers provided very positive and constructive feedback. In addition, R1 raised several important considerations about our proposed evidential regularizer. We address R1's concerns, point-by-point, as part of the rebuttal (3.2a and 3.2b). We also note that, as part of our original submission, we provide a complete ablation analysis (Sec. 4.1 and Sec. S2.1.3) that demonstrates the utility and necessity of our proposed regularizer. In response to R1's concerns regarding conflated aleatoric and epistemic uncertainties, in our rebuttal we provide new results from the exact experiment they requested. As is shown, our approach captures high aleatoric uncertainty in regions of high noise within the data distribution while maintaining low epistemic uncertainty in this domain. Critically, in this experiment epistemic uncertainty only starts to increase in OOD regions. These results further support our claim that aleatoric and epistemic uncertainties can be disentangled using our method. We believe the requested experiment is very valuable and will include these results in our updated manuscript to address this key consideration pointed out by R1. Regarding R1's request for additional performance statistics on depth experiments, we are also happy to include all of these metrics (in addition to the metrics already provided, which include RMSE) in the updated manuscript to further strengthen our results. Please note that these requested metrics can all be computed directly from our existing results without running any additional experiments. 

We believe that our response addresses all reviewer concerns while further strengthening the significance of our results.

Thank you very much for your consideration.

Regards,
Authors of Deep Evidential Regression


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
